Solving the unique continuation problem for Schr\"odinger equations with low regularity solutions using a stabilized finite element method

In this paper, we consider the unique continuation problem for the Schr\"odinger equations. We prove a H\"older type conditional stability estimate and build up a parameterized stabilized finite element scheme adaptive to the \textit{a priori} knowledge of the solution, achieving error estimates in interior domains with convergence up to continuous stability. The approximability of the scheme to solutions with only $H^1$-regularity is studied and the convergence rate for solutions with regularity higher than $H^1$ is also shown. Comparisons in terms of different parameterization for different regularities will be illustrated with respect to the convergence and condition numbers of the linear systems. Finally, numerical experiments will be given to illustrate the theory.

==> deleted.tex <==
\begin{proof}[Proof of \thref{ultraweak}]
\color{red}
Recall the estimate in \thref{ultraweak}
\begin{equation}\label{ultraweakestimate}
    \begin{aligned}
        ||u||_{B_2}\le & C(P)(||u||_{B_1}+||\mathcal{L}u||_{H^{-2}(\Omega)})^\kappa(||u||_{\Omega}+||\mathcal{L}u||_{H^{-2}(\Omega)})^{1-\kappa}.
        \end{aligned}
    \end{equation}
We only need to prove the estimate for $u\in H^2(\Omega)$ then use the density argument to validate it for all $u\in L^2(\Omega)$. Take the geometry and the cut-off function $\psi$ the same as in the previous proof and let $w$ defined by the solution of
\begin{equation}
       \left\{\begin{array}{rlc}
        -\Delta w+Pw & =\psi \mathcal{L}u & \texttt{in $\Omega$,}   \\
        \partial_n w+iw & =0 & \texttt{on $\partial \Omega$.}
        \end{array}\right.
    \end{equation}
\textbf{Step1.} We show that actually $||w||_\Omega \le ||\mathcal{L}u||_{H^{-2}(\Omega)}$. Consider the variational formulation
 \begin{equation*}
        \int_\Omega \nabla w\cdot \nabla \bar{v}dx+\int_\Omega Pw\bar{v}dx - i\int_{\partial\Omega}w\bar{v}dS=\int_\Omega \psi \mathcal{L}u \bar{v}dx.
    \end{equation*}
Let $\phi\in C_c^\infty(\Omega\backslash\bar{B_4})$ be another cut-off function that takes value $1$ near the boundary of $\Omega$, and by testing the above formula by $\phi w$ and take the imaginary part we obtain $w=\partial_nw=0$ at the boundary $\partial\Omega$. Therefore $w\in H^2_0(\Omega)$. Moreover, we have 
\begin{equation*}
    \text{supp}(w)\subset B_4.
\end{equation*}
This is because we could apply the unique continuation principle for the Cauchy data on $\partial\Omega$ to the domain $\Omega\backslash\bar{B_4}$. Then by considering a similar problem again
\begin{equation}
       \left\{\begin{array}{rlc}
        -\Delta W+PW & = w & \texttt{in $\Omega$,}   \\
        \partial_n W+iW & =0 & \texttt{on $\partial \Omega$,}
        \end{array}\right.
    \end{equation}
we obtain that $W\in H^2_0(\Omega)$. This gives an important estimate
\begin{equation*}
    ||w||_{\Omega}^2 = \int_\Omega w\mathcal{L}Wdx \le C(P)||\mathcal{L}w||_{H^{-2}(\Omega)}||W||_{H^2(\Omega)}\le C(P)||\mathcal{L}w||_{H^{-2}(\Omega)}||w||_\Omega,
\end{equation*}
where the last inequality is from the elliptic regularity (\ref{regularity}). Finally we have
\begin{equation*}
    ||\mathcal{L}w||_{H^{-2}(\Omega)} = \sup_{v\in H^2_0(\Omega)}\frac{\int_\Omega \mathcal{L}u(\psi v)dx}{||v||_{H^2_0(\Omega)}}\le ||\mathcal{L}u||_{H^{-2}(\Omega)}.
\end{equation*}
\textbf{Step 2.} We finish the proof by a similar approach as in the proof of \thref{co2}. Take $v=u-w$, then $\mathcal{L}v$ vanishes in $B_3$. Thus we have
\begin{equation}
        ||v||_{B_2}\le C(P)||v||_{B_1}^\kappa ||v||_{B_3}^{1-\kappa}.
    \end{equation}
    This estimate can be obtained by using \thref{L2error}. Then we have
    \begin{equation*}
        \begin{aligned}
            ||v||_{B_2}&\le C(P)||v||_{B_1}^\kappa ||v||_{B_1}^{1-\kappa}\\
            &\le C(P)(||u||_{B_1}+||w||_{B_1})^\kappa (||u||_{B_3}+||w||_{B_3})^{1-\kappa}\\
            &\le C(P)(||u||_{B_1}+||\mathcal{L}u||_{H^{-2}(\Omega)})^\kappa (||u||_{B_3}+||\mathcal{L}u||_{H^{-2}(\Omega)})^{1-\kappa}.
        \end{aligned}
    \end{equation*}
Finally, by the above bound for $||v||_{B_2}$ and the bound for $||w||_\Omega$ in Step 1, we have
\begin{equation*}
    \begin{aligned}
        ||u||_{B_2} \le ||v||_{B_2} + ||w||_{B_2}\le C(P)(||u||_{B_1}+||\mathcal{L}u||_{H^{-2}(\Omega)})^\kappa (||u||_{B_3}+||\mathcal{L}u||_{H^{-2}(\Omega)})^{1-\kappa}.
    \end{aligned}
\end{equation*}
    
\end{proof}
